Towards Applying Powerful Large AI Models in Classroom Teaching: Opportunities, Challenges and Prospects

This perspective paper proposes a series of interactive scenarios that utilize Artificial Intelligence (AI) to enhance classroom teaching, such as dialogue auto-completion, knowledge and style transfer, and assessment of AI-generated content. By leveraging recent developments in Large Language Models (LLMs), we explore the potential of AI to augment and enrich teacher-student dialogues and improve the quality of teaching. Our goal is to produce innovative and meaningful conversations between teachers and students, create standards for evaluation, and improve the efficacy of AI-for-Education initiatives. In Section 3, we discuss the challenges of utilizing existing LLMs to effectively complete the educated tasks and present a unified framework for addressing diverse education dataset, processing lengthy conversations, and condensing information to better accomplish more downstream tasks. In Section 4, we summarize the pivoting tasks including Teacher-Student Dialogue Auto-Completion, Expert Teaching Knowledge and Style Transfer, and Assessment of AI-Generated Content (AIGC), providing a clear path for future research. In Section 5, we also explore the use of external and adjustable LLMs to improve the generated content through human-in-the-loop supervision and reinforcement learning. Ultimately, this paper seeks to highlight the potential for AI to aid the field of education and promote its further exploration.

==> OK/approach.tex <==
\section{Scenarios and Approaches}
In this section, we describe the federated scenarios that distributed users query the LLMs with similar (but not exact the same) questions. We identify two types of questions and discuss them in details.

\subsection{Notations and Concepts of LLMs}
\chenyou{probably we can ignore this}
\textbf{Chain-of-Thought (CoT)}~\cite{wei2022chain} is a series of generated intermediate reasoning texts that can be added to the original prompts. CoT is proposed for enhancing the capability of language models to perform various reasoning tasks by allowing LLMs to decompose complex problems into intermediate steps that could be solved well step-by-step. Chain-of-thought prompting, i.e. prompting LLMs with CoT, is a simple and practical method for improving the reasoning tasks readily with no additional efforts of tuning the original LLMs. CoT prompting has shown improved reasoning results on arithmetic, commonsense, and symbolic reasoning tasks. 

\textbf{Self-Consistency (SC)}~\cite{wang2023selfconsistency} is a decoding strategy that enhances language model reasoning with voting ensemble. SC first samples a diverse set of answers as reasoning paths of a question, rather than only the greedy path. By exploring multiple paths, SC is capable of identifying the most consist answer as the final answer by majority voting, i.e., the most voted answer of the LLM is taken as the final answer. Compared with a single-path reasoning, SC ensembles answers to improve accuracy and filters out noises or outliers. 
SC has also been widely explored in reasoning and QA tasks~\cite{wang2023selfconsistency}.
%The proposal of self-consistency represents a significant milestone in the ongoing effort to improve the reasoning ability of language models, as it has since been widely recognized as a crucial method to enhance their performance.

\textbf{Majority voting(MV)}\cite{Ongaro2014Consensus} is a commonly used method in statistical decision theory that involves aggregating the opinions or decisions of multiple individuals or models, typically by selecting the option with the highest frequency of agreement among the voters.


\subsection{Synonymous Questions with Same Parameters (SP-questions)}
We consider a cloud-based LLM system which accepts queries from distributed users. The first practical user scenario that we consider is as follows. Given a user query, we can retrieve from the cloud database several \textbf{synonymous questions with same parameters (SP-questions)}. 
% The cloud-deployed system retrieves from the database and finds several \synm but rephrased questions with same parameters.  

%{\sethlcolor{cyan}\hl{ALL: we should discuss how to describe this online. Place here for remind.}}
% For example,\\
% \emph{Q1:"If a farmer has a certain number of chickens and rabbits in a barn, and there are a total of 32 heads and 100 feet, how many chickens and how many rabbits does the farmer have?"
% A1:"The farmer has 24 chickens and 8 rabbits."(wrong)
% Q2:"In a barn, there are a certain number of chickens and rabbits that have a total of 32 heads and 100 feet.  how many of each animal are in the barn?"
% A2:"Let x = the number of chickens and y = the number of rabbits. We can set up the following system of equations:x + y = 32  (heads), 2x + 4y = 100  (feet) , Solving this system of equations, we get x = 20 and y = 12.Therefore, there are 20 chickens and 12 rabbits in the barn.(wrong)"}


% For another example, 
% \emph{Q1:"James writes a 3-page letter to 2 different friends twice a week.  How many pages does he write a year?"
% A1:"James writes 3 pages to 2 different friends twice a week, which is 24 pages a month and 288 pages a year."(wrong)
% Q2:"If James writes a 3-page letter to two different friends twice per week, what is the total number of pages he produces every year?"
% A2:" James writes two 3-page letters twice per week.There are 52 weeks in a year. Therefore, James produces a total of 312 pages every year (2 x 3 x 52 = 312)."(wrong)}
\begin{table}[ht]%!htbp
    \centering 
    \vspace{-5pt}
    \caption{Examples of \synm SP-questions and answers.  }
    % \begin{tabular}{l}
    \begin{tabular*}{\hsize}{@{}@{\extracolsep{\fill}}l@{}}
         \toprule
         \emph{Example1:}\\
         \midrule
         \emph{\textbf{Q1:} ``If a farmer has a certain number of chickens and rabbits in a barn, and }\\\emph{there are a total of $32$ heads and 100 feet, how many chickens and how many}\\\emph{rabbits does the farmer have?''}\\
         \emph{\textbf{A1:} ``The farmer has $24$ chickens and 8 rabbits.''} \textcolor{red}{(wrong)}\\
         \midrule
         \emph{\textbf{Q2:} ``In a barn, there are a certain number of chickens and rabbits that have}\\\emph{a total of $32$ heads and $100$ feet.  how many of each animal are in the barn?''}\\
         \emph{\textbf{A2:} ``Let $x=$ the number of chickens and $y=$ the number of rabbits. We can}\\\emph{ set up the following system of equations:$x + y = 32  (heads)$, $2x + 4y = 100$}\\\emph{ (feet), Solving this system of equations, we get $x = 20$ and $y = 12$.Therefore,}\\\emph{ there are $20$ chickens and $12$ rabbits in the barn.''} \textcolor{red}{(wrong)}\\
         \toprule
         \emph{Example2:}\\
         \midrule
         \emph{\textbf{Q1:} ``James writes a $3$-page letter to $2$ different friends twice a week.How many}\\\emph{pages does he write a year?''}\\
         \emph{\textbf{A1:} ``James writes $3$ pages to $2$ different friends twice a week, which is $24$ pages} \\\emph{ a month and $288$ pages a year.''} \textcolor{red}{(wrong)}\\
         \midrule
         \emph{\textbf{Q2:} ``If James writes a $3$-page letter to two different friends twice per week,what} \\\emph{ is the total number of pages he produces every year?''}\\
         \emph{\textbf{A2:} ``James writes two $3$-page letters twice per week. There are $52$ weeks in a }\\\emph{year. Therefore, James produces a total of $312$ pages every year($2 * 3 * 52=312$).''} \\ \textcolor{red}{(wrong)}\\
        \bottomrule
    \end{tabular*}
    \label{tab:SP-question-example}
\end{table}%三线表结束

For complex reasoning tasks, the LLMs may provide unreliable answers to the questions. We provide two failure cases in Table.~\ref{tab:SP-question-example}. We found that in both examples, Q1 and Q2 are \synm while each of them gets a wrong answer from LLM. We summarize the difficulties of tackling the SP-questions as follows: 
%\hl{WHAT? No ground truth answer? Or some rephrased context is difficult for LLMs to understand>? Single zero-shot is hard?  Summarize them.}\\
% 1.大部分LLMs对推理的问题的准确度较低
% 2. LLMs对于包含多个步骤复杂的问题理解能力较差
% 3. 使用CoT可以提升准确率，但是特定问题进行特定的prompt较为困难
% 4. 使用Self-consistency可以增加问题的准确率，但是成本很高且不能复用
\begin{enumerate}[noitemsep,leftmargin=*]
\item Most LLMs have unsatisfying accuracy in solving reasoning problems in zero-shot way, i.e.,  prompting the LLMs with questions directly without giving other information.
\item LLMs tend to under-perform when understanding complex problems involving multiple reasoning steps, such as the arithmetic problems given above.
% \item While using CoT can enhance accuracy, it can be challenging to tailor specific prompts for particular problems. 
% %\hl{Done:Did we mention CoT? If not, we should describe CoT.}
% \item Implementing self-consistency can increase problem accuracy, but it comes at a high cost and cannot be reused. 
%\hl{DoneDid we mention SC ? If not, we should describe CoT.}
\end{enumerate}

Thus, our task is to \emph{fully explore the SP-questions as a federation which can enhance the answer quality together}, instead of dealing them separately. To this end, we propose a technique named \textbf{Fed-SP-SC} (Federated SP-questions with Self-Consistency) for answering the questions with the self-consistency technique mentioned above. Fed-SP-SC can improve the zero-shot accuracy of the answers by eliciting answers from multiple \synm questions and make a majority vote to disclose the most likely answer. 

 % 我们通过使用prompt查询数据库中的数据，以匹配数据库中的问题，将本次用户的prompt进行回答并结合数据库中查询到的same questions same parameters进行self-consistency。最后将结果反馈给用户，本次用户的prompt和生成的回答会放入数据库中（为了后文的Fed-DP）并更新self-consistency中的多数投票数据。
%原翻译
%\hl{Xiangyang:"This paragraph is a direct translation of the above comment."}\\
Concretely, we query the database using the user's prompt to match SP-questions in the database. Note that here we assume we can retrieve the SP-questions which are just rephrased with \synm and same parameters.

Next, we generate the answers with LLMs by zero-shot prompting. For SP-questions, these answers are presumably same. Assuming that we have generated a total of \emph{n} 
answers of \synm questions during the Fed-SP-SC process, we can ensure the consistency with SC procedure, i.e., we make a majority vote and select the most voted answer $A^{SC}$ as the final answer of all SP-questions, as below.
\begin{equation}
    A^{SC} \leftarrow \argmax_{A \in \mathcal{A}} \sum \mathbf{1}[A==A_i], \ \ 
\forall i=1,...,n  \ .
\end{equation}

Intuitively, the majority voting filters out outliers and noisy rephrased questions. In addition,
the most voted answer is the agreement of multiple reasoning paths from multiple rephrased SP-questions, thus is more likely to be better than a single prompted answer decoded from a single reasoning path.  

In our experiments, we demonstrate that Fed-SP-SC achieves a 17.5\% improvement in accuracy on the GSM8K dataset and a 14\% improvement on the SVAMP dataset in Table \ref{tab:Fed_SP_SC_result}. In a practical system, we can further store these user prompts and the SC-selected answer back into the database.

%\hl{Done: Here should we explain why most voted answer is better? Can we find some sentences in original SC paper and rephrase some explanation here} 

% In the paper proposing Self-consistency~\cite{wang2023selfconsistency}, the author compares the effectiveness of several aggregation strategies through experimentation and finds that using the "unweighted sum" approach (i.e. majority voting) produces results that are very similar to those obtained through calculating the exact "normalized weighted sum" approach, but with a lower computational cost. Therefore, majority voting can be used as an approximate solution in practical applications.
% In a practical system, we can further store these user prompts and the SC-selected answer back into the database.

%\hl{Done:  Can we add a figure here. Use Chicken-rabit example maybe. We show three or five rephrased SP-questions.  Three of them correct, 1 wrong and another one wrong. Then add a histogram showing 3:1:1 voting. So that correct answer is selected. 
%}
\begin{figure}[ht]
%\vspace{-8pt}
\begin{center}
\includegraphics[clip, trim=0 20 0 0, width=0.9\textwidth]{figures/Fed-SC5.pdf}
\end{center}
\vspace{-8pt}
%当接收到用户的query时，LLMs会从数据库中检索SP问题，当检索到SP问题后，便会调用历史投票结果与用户query的回答一起进行self-consistency.
% highlight section backup: The LLM then generates the answers with zero-shot prompting for each SP-question and the new query, then calls for majority voting to ensure self-consistency over SP-questions.
\caption{The illustration of performing Fed-SP-SC for answering \synm SP-questions. $(A \rightarrow B)$: When receiving the user's query, the LLM retrieves \synm SP-questions from the centralized database. $(B \rightarrow C)$: The LLM generates the answers with zero-shot prompting for the query and combines the retrieved SP-questions' answers from the database for a majority vote to ensure self-consistency. $(C \rightarrow D)$: The most voted answer is returned to the user as the best answer. The database could store the query and answer pair back to the database, caching for later retrieval. This procedure can grow the database quickly by gathering distributed user queries. }
\label{fig:Fed-SC}
\vspace{-6pt}
\end{figure}



% 润色后 
%\hl{Xiangyang:"This paragraph has been polished by chatgpt, and there may be deviations in the meaning to be expressed!!!"} \\
% To improve the accuracy of the answers, we initiate a process where the user's input prompt is queried against the database to retrieve matching questions. The retrieved questions are then used to generate an answer, which is then used to performed self-consistency with the same questions with same parameters used for querying the database. This self-consistency process is performed to ensure that the generated answer is more reliable and more accurate. The resulting answer is presented to the user, and both the user's prompt and the generated answer are stored in the database for potential future use in  Fed-DP. Finally, the majority voting data obtained during the self-consistency process is updated to improve the accuracy in same and similar questions.


 \subsection{Synonymous questions with Different Parameters (DP-questions)}
We now describe the second scenario which is named \textbf{\synm questions with different parameters (DP-questions)}, which is broader and more practical. 
Based on the user query question, the cloud-deployed system searches and retrieves from the database for questions with same meanings but may have different parameters.  
%{\sethlcolor{cyan}\hl{ALL: we should discuss how to describe this off-line. Place here for remind.}}

% \hl{Tianqi: the Q1 and Q2 questions format look not nice. Can we make them look better.}
DP-questions are more practical yet harder than SP-questions as the question parameters retrieved from the database are different. We show two exemplary questions Q1 and Q2 below which have the same meaning yet with different parameters \emph{heads} and \emph{feet} in Table \ref{tab:DP-question-example}. 
% \emph{Q1:"If a farmer has a certain number of chickens and rabbits in a barn, and there are a total of 32 heads and 100 feet, how many chickens and how many rabbits does the farmer have?"\\
% Q2:"A farmer has a total of 20 chickens and rabbits in his barn. If the total number of legs in the barn is 56, how many chickens and how many rabbits are in the barn?"} 
\begin{table}[!ht]%!htbp
    \centering 
    % \setlength{\abovecaptionskip}{0.01cm}
    \caption{Two examples of DP-questions. \emph{Q1} and \emph{Q2} are synonymous but with different question parameters.
}
    \begin{tabular*}{\hsize}{@{}@{\extracolsep{\fill}}l@{}}
         \toprule
         The specific description of \emph{Q1} and \emph{Q2:}\\
         \midrule
         \emph{\textbf{Q1: } ``If a farmer has a certain number of chickens and rabbits in a barn and},\\\emph{there are a total of 32 heads and 100 feet, how many chickens and how many}\\\emph{rabbits does the farmer have?''}\\
         \emph{\textbf{Q2: } ``A farmer has a total of 20 chickens and rabbits in his barn. If the total}\\\emph{number of legs in the barn is 56, how many chickens and how many rabbits} \\\emph{are in the barn?''}\\
        \bottomrule
    \end{tabular*}
    \label{tab:DP-question-example}
\end{table}%三线表结束

Note that tackling DP-questions would face all the difficulties of SP-questions, and would have additional obstacles as summarized below: 
% \hl{Xiangyang:"a new idea For Fed-SP, we can put some ground truth in the database, such as splicing together the QA in the benchmark data set as the initial data"}
\begin{enumerate}%[noitemsep,leftmargin=*]
\item There is no uniform ground-truth for DP-questions in the database, since each one has different parameters. 
%and the improvement of accuracy needs to be done by LLMs themselves(Corresponding to the idea above)
\item Similarly, we cannot apply self-consistency (SC) directly to improve accuracy due to different parameters.
%\item While using CoT can enhance accuracy, it can be challenging to tailor specific prompts for particular problems.
\item If we apply Chain-of-Thought (CoT) together to the original questions as enhanced prompts, we cannot guarantee the correctness of the CoT. Incorrect CoT may even harm the answering accuracy.
\end{enumerate}


To tackle the above challenges, we propose the \textbf{Federated questions of Different Parameters with Chain-of-Thought} (Fed-DP-CoT) technique to leverage existing answers of DP-questions in CoT forms to improve new query answering. 
\begin{figure}[!ht]
%\vspace{-8pt}
\begin{center}
\includegraphics[clip, trim=0 60 0 0, width=0.9\textwidth]{figures/Fed-CoT-picture4.pdf}
\end{center}
\vspace{-5pt}
% 当LLMs没有检索到SP问题时，便从数据库中检索DP问题，检索到DP问题后，将DP问题的问题答案拼接起来，并加上伪标签警告作为新prompt的前缀。最后，我们加上用户query后，得到完整的 CoT prompt。
% highlight section backup:The system selects the more relevant ones and produce answers as pseudo-labels.
\caption{The illustration of performing Fed-DP-CoT. 
$(A \rightarrow B)$: DP-questions are firstly retrieved from the centralized user query  database. $(B \rightarrow C)$: The system selects SP-questions with consistent answers after applying Fed-SP-SC as DP-questions and retrieves consistent answers as ``pseudo-labels''. $(C \rightarrow D)$: The system concatenates questions and pseudo-labels, adds a pseudo-label disclaimer such as ``The examples may have errors.'' after, and finally appends the original user query and Zero-Shot-CoT to form the complete CoT prompt. }
\label{fig:Fed-CoT}
\vspace{-6pt}
\end{figure}





%\hl{Xiangyang: Please describe here how to perform Fed-CoT. Apply zero-shot first individually multiple-times? Then apply SC and MV to get psuedo-label? And aggregate all Fed-DP questions as CoT?  Note that you can use psuedo-label to describe that the majority voted answer is not exactly the ground-truth answer.  Maybe you have time to carry on ablation about using true answer later.}
% 当接受到用户的提问时，LLMs会检索数据库里面的数据，如果数据库中没有相同的问题(SP)，便开始执行Fed-CoT。我们会匹配数据库中相似度最高的一个或几个问题(这些问题是由Fed-SC过程中经过Self-consistency多数投票生成的伪标签，也就是说并没有ground truth)，通过将这些问题和回答拼接起来，并在末尾加上"The example given above may have some errors"作为DP问题的CoT prompt。我们通过研究发现，即使参数不同，也可以增加问题的准确性。[初稿]

When a user starts querying the cloud-based LLM service, the cloud system performs query-question retrieval first. The system matches several questions with the highest similarity in the database. Generally, these  the retrieved questions are of different parameters (DP-questions). We design the system  to perform Fed-DP-CoT for understanding DP-questions.


We consider a practical case that these DP-questions have \emph{pseudo-labels} generated by self-consistency majority voting in the Fed-SP-SC processes.
We call these labels ``pseudo-labels'' as they are not actual ground-truth labels.



% 具体来说，我们将这些DP-questions的问题和答案拼接成一段prompt，如问题1-回答1-问题2-回答2...,然后在这段prompt后加上“The example given above may have some errors”(这是为了让大语言模型意识到这些prompt只是伪标签). 最后将整段prompt作为前缀加上用户query的问题作为我们最终的prompt来让LLMs回答。


Then we utilize these DP-questions with pseudo-labels together as CoT for the original query-question. 
To be specific, we concatenate DP-questions with their answers as a single prompt, followed by the error disclaimer
%, such as Question 1-Answer 1-Question 2-Answer 2..., and append the phrase 
``The examples given above may contain errors , please think more carefully. '' at the end of this prompt  as the complete prompt.
%(\hl{this is CoT or Prompt? Answer: CoT refers to the process of thinking before giving an answer. Prompt refers to the content of the conversation with LLMs, so here I prefer to use prompt}). 
The error disclaimer reminds the LLMs that the answers in CoT are pseudo-labels and could be incorrect. We found this simple practice can boost performance by approximately 2\%.
% We take the CoT together with the original query as the final prompt for answer.
Finally, we use the entire disclaimed CoT as a prefix to the user's query prompt for the LLMs to provide the final answer.



\subsection{Available tools for LLM implementations}
In practice, we utilized the OpenAI's API~\footnote{https://platform.openai.com/docs/models} text-davinci-002 and text-davinci-003. We selected text-davinci-003 for the GSM8K dataset as text-davinci-002 performed very poorly. Similarly, we used text-davinci-002 for the SVAMP dataset as text-davinci-003 had an overly high accuracy rate on this dataset.  

==> OK/experiments.tex <==
\section{Experiment}
\label{sec:exp}

We evaluate our proposed \textbf{Fed-SP-SC} and \textbf{Fed-DP-CoT} methods on benchmark datasets with simulated user scenarios such that SP- and DP-questions are retrieved to improve over standalone question answering.

We compare our methods with \emph{Zero-Shot-CoT}~\cite{brown2020language}, which refers to adding \emph{``Let's think step by step.''} to prompt as a composite prompt, such as ``[Question] A:Let's think step by step.'' 
% In this section, we elaborate on the experimental settings and analyze the results in details.

\subsection{Datasets}
\label{sec:dataset}

\textbf{Grade School Math (GSM8K)} is a math dataset with 7,473 training and 1,319 testing examples of grade-school-level word problems\cite{Cobbe2021TrainingVT}. These math problems typically require two to eight calculation steps to arrive at a final answer, as shown in Fig.\ref{fig:Fed-SC}. GSM8K is widely used as a benchmark dataset for testing the arithmetic and commonsense reasoning capacities of LLMs~\cite{huang2022large, kojima2023large}.
%It should be noted that the sample size of this dataset is relatively small and may not cover all possible math word problems, but it is still a valuable dataset for evaluating the performance of NLP models.

% \textbf{Simple Variations on Arithmetic Math word Problems (SVAMP)} This dataset is a challenge dataset for simple arithmetic math word problems (MWPs) based on natural language processing (NLP), introduced by Patel et al\cite{patel2021nlp}.The dataset primarily contains challenge data for evaluating a model's performance in solving simple arithmetic MWPs. The SVAMP dataset consists of approximately 6,000 samples, each containing a short natural language narrative that describes a state of the world and poses a question about some unknown quantities. Each sample covers a simple arithmetic problem that requires reasoning and computation to arrive at the correct answer. 
% The dataset's purpose is to test the performance of natural language processing models in solving simple arithmetic math word problems and provide a benchmark test set for comparing the performance of different models for researchers and developers. The SVAMP dataset is designed to provide challenging samples that can test a model's reasoning and computational abilities and help improve and optimize the performance of NLP models.

\textbf{Simple Variations on Arithmetic Math word Problems (SVAMP)} is a dataset of simple arithmetic math word problems~\cite{patel2021nlp} with around 6,000 samples. Each data instance has a short story and a question about unknown quantities. SVAMP provides a benchmark test set for comparing the textual understanding and reasoning abilities of LLMs, which is widely compared in recent studies~\cite{patel2021nlp, wei2022chain, wang2023selfconsistency}.

% \subsection{Evaluation Metrics}
% \label{sec:evaluation_metrics}


In practice, we utilized the OpenAI's API~\footnote{https://platform.openai.com/docs/models} text-davinci-002 and text-davinci-003. We selected text-davinci-003 for the GSM8K dataset as text-davinci-002 performed very poorly. Similarly, we used text-davinci-002 for the SVAMP dataset as text-davinci-003 had an overly high accuracy rate on this dataset.  

 
%\subsection{Results and Analysis}

\subsection{Results of Fed-SP-SC}
\label{sec:fed-sp-sc_result}






% 在上表中，我们测试了将同一个问题的不同问法得出结果后进行self-consistency后的准确度。
% 在数据方面，我们使用GSM8K和SVAMP两个算术推理数据集来进行实验。用于self-consistency的相同意思的几个问题，我们使用GPT3和GPT3.5来生成相同的问题，通过" Rephrase in 4 ways:"(question needs to be rephrased )" "逐个生成。
% 在实验中，我们使用GPT3作为实验的语言模型。在GSM8K数据集中我们使用了text-davinci-003的接口；因为SVAMP数据集的难度较简单，因此我们采用了text-davinci-002接口来完成测试。( GPT-3 (Brown et al., 2020) with 175-billion parameters. We use two public engines code-davinci001 and code-davinci-002 from the Codex series (Chen et al., 2021) to aid reproducibility; )
% 进行测试时，我们以"Let's think step by step"作为prompt进行测试。
% 从表格中的结果可以发现，通过聚合多个同义问题进行self-consistency可以提升大语言模型的准确率。同义问题的质量越好，带来的提升也越大(可以看到GPT3.5所生成的同义问题带来的提升大于GPT3的)

As a kind reminder, in the following discussions, \textbf{SP-questions} stand for \emph{a set of rephrased \synm questions with same parameters.} Differently, \textbf{DP-questions} stand for \emph{a set of rephrased \synm questions with different parameters. }
We now describe the experiment procedures shown in Fig.~\ref{fig:image}.

[\textbf{SP-questions generation}]. We first generate four SP-questions for each of the original question with both OpenAI GPT-3~\cite{brown2020language} and GPT-3.5~\cite{ouyang2022training}, respectively. Concretely, we add each original question a same prompt prefix \textit{``Rephrase in 4 ways: [ORIGINAL QUESTION]''}, then we collect the generated answers.

[\textbf{SP-questions answering}].
We query the cloud-deployed LLM for answering rephrased questions generated as above.
Specifically, we obtain the improved Zero-Shot-CoT answering with the magic sentence \textit{``Let's think step by step''} as the prompt. 

% Then we utilize the GPT-3 text-davinci-003 API name\footnote{https://platform.openai.com/docs/models}) as the LLM interface for answering SP-questions of GSM8K dataset, and the text-davinci-002 interface for answering SP-questions of SVAMP dataset for saving budget\hl{Done: SVAMP dataset is less challenging than GSM8K, therefore different APIs are used for these datasets.}. We add the zero-shot answering with the magic sentence \textit{"Let's think step by step"} as the prompt~\cite{brown2020language}\hl{Done: add the cite here, who first proposes think step-by-step?} to generate improved standalone answers. 


We first examine the performance of our proposed Fed-SP-SC which deals with SP-questions with the Self-consistency technique. 
We conducted experiments on GSM8K and SVAMP and report the results below.


\begin{figure}[ht]
\centering
\includegraphics[width=1\textwidth]{figures/Fed-SC-Flow-chart.pdf}
\caption{The experiment of Fed-SP-SC contains five steps: (1) Load the GSM8K and SVAMP datasets as our benchmark and extract the questions and answers in the dataset; (2) Add each original question a same prompt prefix ``Rephrase in 4 ways: [QUESTION]'' to generate SP-questions; (3) Prompt both the original and rewritten questions to the LLMs to obtain their respective answers; (4) Use the majority vote for self-consistency;  (5) Get the answer generated by Fed-SP-SC and compare it with the answer in the dataset to determine the accuracy rate.}
\label{fig:image}
\end{figure}


\begin{table}[ht]
\caption{Fed-SP-SC results}
\label{tab:Fed_SP_SC_result}
\centering
\begin{tabular}{l|c | c | c}
% \caption{Result}
\toprule
Data\textbackslash{}Method & Zero-Shot-CoT & \begin{tabular}[c]{@{}c@{}}Fed-SP-SC \\ (GPT-3 Gen.)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Fed-SP-SC \\ (GPT-3.5 Gen.)\end{tabular} \\ 
\toprule
\multicolumn{1}{c|}{GSM8K} & \multicolumn{1}{c|}{52.5\%} & \multicolumn{1}{c|}{63\%}  & \multicolumn{1}{c}{70\%}    \\
\multicolumn{1}{c|}{SVAMP} & \multicolumn{1}{c|}{78\%} & \multicolumn{1}{c|}{87\%}  & \multicolumn{1}{c}{92\%}  
\\ 
\toprule
\end{tabular}
\end{table}


We show accuracy of self-consistency after obtaining results from different phrasings of the \synm question on GSM8K and SVAMP in Table~\ref{tab:Fed_SP_SC_result}. 
We have the following observations.

\begin{itemize}[noitemsep,leftmargin=*]
\item \emph{Fed-SP-SC can improve answering accuracy} of LLMs by federating multiple SP-questions through self-consistency. 
\item \emph{Fed-SP-SC(GPT-3.5 Gen.) performs best on the GSM8K and SVAMP datasets,} improved the performance by $17.5\%$ and $14\%$ on the GSM8K and SVAMP datasets, respectively.
\item \emph{The quality of the \synm questions can affect the accuracy significantly}, as seen in the larger improvement from the \synm questions generated by GPT-3.5 compared to GPT-3.
\end{itemize}
% We show accuracy of self-consistency after obtaining results from different phrasings of the same question on GSM8K and SVAMP in Table~\ref{tab:res_consistency}. 
% We have the following observations.
%\begin{itemize}[noitemsep,leftmargin=*]
%\item \emph{For datasets.} We conducted experiments on two arithmetic reasoning datasets, GSM8K and SVAMP. For the same meaning questions used for self-consistency, we used GPT-3 and GPT-3.5 to generate four rephrased questions for each original question through the \textit{"Rephrase in 4 ways"} function.

%\item \emph{For experiments.} We used the GPT-3 language model. We used the text-davinci-003 interface for the GSM8K dataset, and the text-davinci-002 interface for the SVAMP dataset, as it was less difficult. We used the public engines code-davinci001 and code-davinci-002 from the Codex series to ensure reproducibility.We conducted the tests using \textit{"Let's think step by step"}as the prompt. 
%\item \emph{For results.} The results from the table show that the accuracy of large language models can be improved by aggregating multiple same-meaning questions through self-consistency. The quality of the same-meaning questions can affect the degree of improvement, as seen in the larger improvement from the same-meaning questions generated by GPT-3.5 compared to GPT-3.
%\end{itemize}




%\begin{itemize}[noitemsep,leftmargin=*]
%\item \emph{DQC-Rank performs best in per-class accuracy (PAcc)}. Due to the class imbalance, other approaches bet more on the majority class (neutrality) thus have larger QAccs. 
%\item \emph{DQC-Rank consistently outperforms in Gain and SR}, leading the second place by around 15\%. 
%\item \emph{DQC-Rank has a slightly larger max drawdown (MDD)}, as it is designed to capture large movements. Still, DQC-Rank strikes a good balance between sensitivity and volatility (high SR) by better capturing the rising opportunities of the stocks.   
%\end{itemize}



\subsection{Results of Fed-DP-CoT}
\label{sec:fed_cot_result}

\begin{figure}[ht]
\centering
\includegraphics[width=1\textwidth]{figures/Fed-CoT-Flow-chart.pdf}
\caption{The experiment of Fed-DP-CoT contains five steps:(1) Form a new test set by rephrasing the questions using different parameters in the benchmark manually and providing answers; (2) Extract consistent questions and answers in Fed-SP-SC experiment; (3) Add a disclaimer to form the CoT prompt; (4) Add the rephrased questions after the CoT prompt; (5) Prompt LLMs with entire CoT prompt and compared the answers with the rephrased answers for evaluation. }
\label{fig:Fed-DP-CoT-flow-chart}
\end{figure}

% 下面这段文字都总结到上面的figure caption中了

% In Experiment 2, we employed a subset of the problem set used in Experiment 1 to conduct experiments with the text-davinci-003 model on the GSM8K dataset and the text-davinci-002 model on the SVAMP dataset. To improve the accuracy of FedCoT under different parameter settings, we utilized CoT prompts. In the data preparation phase, we manually modified the parameters of the questions in both datasets and simulated different parameter configurations by providing the answers after the parameter changes. Our CoT prompts were generated using synonymous questions from Experiment 1. Self-consistency was employed for majority voting in Experiment 1, and the winning CoT from the majority vote was used as part of our prompt. We concatenated these CoT prompts and added the statement "r “The examples
% given above may contain errors, please think more carefully." to form our prompt. Through our experiments, we demonstrate that FedCoT can improve the accuracy of LLM across the same set of questions with varying parameter settings.

% 实验二中，我们使用实验一中问题的子集进行实验，在GSM8K数据集上我们使用text-davinci-003,在SVAMP数据集上我们使用text-davinci-002,我们通过使用CoT prompt来提升不同参数时FedCoT的准确性。在数据准备阶段，我们通过手动改写GSM8K和SVAMP中问题的参数，并人工给出参数改变后的答案来进行模拟参数不同的状况。我们通过实验一时产生的同义问题来生成我们的CoT prompt，实验一我们使用了Self-consistency进行多数投票，我们使用多数投票中胜出者的CoT作为prompt的一部分，我们将这些CoT拼接，并在拼接后加上“The example given above may have some errors.”作为我们的prompt，经过实验，我们证明了通过使用Fed-CoT也能提升LLM在不同参数的相同问题的准确性。

\begin{table}[htp]
\caption{Fed-DP-CoT results.}
\label{tab:Fed_CoT_result}
\centering
\begin{tabular}{l|c| c| c}
% \caption{Result}
\toprule
Setting\textbackslash{}Method & Zero-Shot-CoT & \begin{tabular}[c]{@{}c@{}}Fed-DP-CoT\\ (GPT-3 Gen.)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Fed-DP-CoT\\ (GPT-3.5 Gen.)\end{tabular} \\ 
\toprule
\multicolumn{1}{c|}{GSM8K} & \multicolumn{1}{c|}{48.3\%} & \multicolumn{1}{c|}{59.2\%}  & \multicolumn{1}{c}{62.5\%}    \\
\multicolumn{1}{c|}{SVAMP} & \multicolumn{1}{c|}{76.7\%} & \multicolumn{1}{c|}{83.3\%}  & \multicolumn{1}{c}{86.7\%}  
\\ 
\toprule
\end{tabular}
\end{table}

We report results of Fed-DP-CoT on GSM8K and SVAMP in Table~\ref{tab:Fed_CoT_result}, and compare with the baseline Zero-Shot-CoT.
% During the experiment, we utilized the text-davinci-003 model to evaluate accuracy on the GSM8K dataset and text-davinci-002 to assess performance on the SVAMP dataset. Our findings indicate that the implementation of Fed-CoT significantly enhances the accuracy of DP-question answering. Specifically, for the question-answering sets generated by GPT-3, we observed a 10.9\% and 6.7\% increase in accuracy on the GSM8K and SVAMP datasets, respectively. Moreover, for the question-answering sets generated by GPT-3.5, the accuracy of GPT-3 improved by 14.2\% on the GSM8K dataset and by 10\% on the SVAMP dataset. In this experiment, we observed a smaller gap between the performance of GPT-3 Gen. and GPT-3.5 Gen. compared to the Fed-SC experiment. We hypothesize that this difference may be attributed to variations in parameters, and also the CoT prompt being less sensitive to the synonymity of the questions.

\begin{itemize}[noitemsep,leftmargin=*]
\item \emph{Fed-DP-CoT can improve the performance.} Compared to Zero-Shot-CoT, CoT Prompt(GPT-3 Gen.) and CoT Prompt(GPT-3.5 Gen.) improve by approximately 10.9\%-14.2\% and 6.6\%-10\% respectively on the datasets GSM8K and SVAMP.
\item \emph{Fed-SP-SC performs better than Fed-DP-CoT.}  The results of Fed-SP-SC (GPT-3 Gen.) and Fed-SP-SC (GPT-3.5 Gen.) on the GSM8K and SVAMP datasets are both higher than Fed-DP-CoT (GPT-3 Gen.) and CoT Prompt (GPT-3.5 Gen.), with an approximate improvement of 5\%.
\item \emph{Less significant performance difference between GPT-3 Gen. and GPT-3.5 Gen. compared to Fed-SP-SC experiment.} The reason for this is the disparity in parameters employed, coupled with the lack of emphasis on synonym usage in the CoT prompt.
\end{itemize}



\subsection{Ablation studies}
\label{sec:ablation}


\begin{figure}[ht]
\centering
\subfloat[GSM8K]{
\includegraphics[width=0.48\textwidth]{figures/Hyper-parameter_Study_GSM8K.png}
\label{fig:GSM8K-ablation-study}
}
\hfill
\subfloat[SVAMP]{
\includegraphics[width=0.48\textwidth]{figures/Hyper-parameter_Study_SVAMP.png}
\label{fig:SVAMP-ablation-study}
}
\caption{Ablation study of choice of sampled reasoning paths.}
\label{fig:ablation-study}
\end{figure}


\textbf{The number of reasoning paths for self-consistency.}
We study the effect of using different number of sampled reasoning paths for Fed-SP-SC (Sec.~\ref{sec:fed-sp-sc_result}) to apply self-consistency. We conduct hyper-parameter search with a subset of the data  for this ablation study due to the limits of accesses of the OpenAI API.  

% We found that the marginal benefits increases until 5, then the benefits decrease from 5-10, and drop over 10. 
We vary the number of sampled reasoning paths of \synm questions from one to nine. Figure \ref{fig:ablation-study} shows that increasing the number of sampled reasoning paths of the \synm questions does not always improve the accuracy of the model. 

In the line chart, as the number of sampled reasoning paths increases from one to five, the accuracy rate gradually increases.
However, when the number of \synm questions exceeds five, the accuracy of the model starts to decrease. 

We speculate that this is because introducing \synm questions also introduces noisy phrases, causing a deviation in the semantic meaning of the original questions. This deviation is particularly evident in synonymous questions generated by GPT-3 (blue lines), while the generation results of GPT-3.5 (orange lines) exhibit stronger robustness.
% 我们对实验一的情况进行了消融实验，并绘制图表。我们发现，使用更多的相同问题进行self-consistency并不总是增加准确率，随着数量增加，在大于5时准确率反而降低。我们推测因为随着相同问题的引入，也产生了部分噪音，使得原来的问题的意义出现了偏差，这在由GPT3生成的同义问题中显得更加明显，而GPT3.5生成的鲁棒性相对更强。


\begin{table}[ht]
\caption{GSM8K disclaimer ablation. }
\label{tab:disclaimer ablation}
\centering
\begin{tabular}{c|c|c|c}
\toprule
Method\textbackslash{}Setting & \begin{tabular}[c]{@{}c@{}}Zero-shot\\-CoT\end{tabular}        & \begin{tabular}[c]{@{}c@{}}Fed-DP-CoT\\ (GPT-3 Gen.) \end{tabular} & \begin{tabular}[c]{@{}c@{}}Fed-DP-CoT\\ (GPT-3.5 Gen.) \end{tabular} \\
\toprule
w/o disclaimer           & 48.3\%           & 57.7\%            & 60\% \\                                   
w/ disclaimer           & NA                 & 59.2\%            & 62.5\%  \\ \toprule                           
\end{tabular}
\end{table}

\textbf{Disclaimer}  We investigate whether the disclaimer is effective of correcting noisy CoTs in this ablation experiment. As Zero-Shot-CoT does not employ pseudo-labels, we do not conduct disclaimer ablation on it. Table \ref{tab:disclaimer ablation} compares the DP-questions answering accuracy with disclaimer or without disclaimer. We observe that the addition of a disclaimer in the questions and answers generated by GPT-3 resulted in an increase in accuracy from 57.7\% to 59.2\% for the Fed-DP-CoT task. Similarly, in the case of questions and answers generated by GPT-3.5, the accuracy increase from 60\% to 62.5\%. These results indicate that the use of a simple disclaimer can potentially improve the accuracy of LLMs by approximately 2\% for the Fed-DP-CoT task. We postulate that the improvement in accuracy may be attributed to the fact that the disclaimer prompts LLMs to be careful of the pseudo-labels and self-examine the reasoning steps.




% 请翻译成英文：“我们观察到，对于GPT3生成的问题集中，disclaimer使得从57.7%上升到59.2%；而再GPT3.5生成的问题集中，从60%上升到62.5。这说明，使用简单的disclaimer大约可以提升Fed-DP-CoT 2%的准确性。我们推测是因为disclaimer让LLMs意识到这些伪标签中并一定是正确答案”

%\textbf{Prompt details.}

% \textbf{Inference speed.}  
% The number of stocks that can be inferred in a second (the higher the faster) are ALSTM (7000), RSR (5000), TFT (1500), DQC-Rank (1200) and DTML (350).
% Notably, our DQC-Rank can process an average of 1200 stocks per second, achieving high-frequency (per-second) prediction for a mid-size market.
% ALSTM and RSR have the advantage of model compactness and runs faster than other Transformer-based models. TFT is slightly faster than our DQC-Rank, as DQC-Rank additionally uses index modality. DTML is slowest as it needs aggregate context from \emph{all} other stocks for individual stock inference.


% 
% We make a grid search of the scaling factors $\alpha_{1,2,3}$ and found $\alpha_1,\alpha_2=0.3$, $\alpha_3=0.2$ to be optimal. We further searched the model dimensions and found the 2-layer multi-head attention with 4 heads and $d_v,d_q,d_\text{model}=64$ to be optimal. For LSTM implementation, we found 1-layer LSTM with hidden size 32 better than more layers or more units.
% We set  , $K=\text{round}(0.1\cdot N)$ and $K'=1$ in our multi-task loss~(\ref{eq:loss_all}).
% We train models with an Nvidia GTX 3090 for 500 epochs, which take about one day to finish. Our DQC-Rank model takes about 1.5G GPU memory for training  with batch size 96. 



% \begin{figure*}
% \centering
% \begin{subfigure}{0.24\textwidth}
%         \includegraphics[clip, trim=30 20 30 30, width=\textwidth]{figures/vis/day_1.png}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.24\textwidth}
%         \includegraphics[clip, trim=30 20 30 30,width=\textwidth]{figures/vis/day_2.png}
% \end{subfigure} 
% \hfill
% \begin{subfigure}{0.24\textwidth}
%         \includegraphics[clip, trim=30 20 30 30,width=\textwidth]{figures/vis/day_3.png}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.24\textwidth}
%         \includegraphics[clip, trim=30 20 30 30,width=\textwidth]{figures/vis/day_4.png}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.24\textwidth}
%         \includegraphics[clip, trim=30 20 30 30,width=\textwidth]{figures/vis/day_5.png}
% \end{subfigure} 
% \hfill
% \begin{subfigure}{0.24\textwidth}
%         \includegraphics[clip, trim=30 20 30 30,width=\textwidth]{figures/vis/day_6.png}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.24\textwidth}
%         \includegraphics[clip, trim=30 20 30 30,width=\textwidth]{figures/vis/day_7.png}
% \end{subfigure} 
% \hfill
% \begin{subfigure}{0.24\textwidth}
%         \includegraphics[clip, trim=30 20 30 30,width=\textwidth]{figures/vis/day_8.png}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.32\textwidth}
%         \includegraphics[clip, trim=30 20 30 30,width=\textwidth]{figures/vis/day_9.png}
% \end{subfigure}
% \caption{Visualization of distributional quantile prediction.}
% \label{fig:dist_visualize}
% \vspace{-10pt}
% \end{figure*}



==> OK/intro.tex <==
\section{Introduction}

\begin{figure}[ht]
%\vspace{-8pt}
\begin{center}
\includegraphics[clip, trim=0 30 0 0, width=0.9\textwidth]{figures/Introduction2.pdf}
\end{center}
\vspace{-8pt}
\caption{A general overview of our approach to dealing with federated synonymous question-answering. Our approach is categorized into two user scenarios: synonymous questions that share the same parameters, and those that have different parameters. When the parameters are the same, we utilize self-consistency to select the most commonly voted answer as the consistent response. However, for cases where the parameters are different, we amalgamate each question's consistent answer to create a Chain-of-Thought, which makes it easier for the LLM to respond to new queries. }
\label{fig:Introduction_image}
%\vspace{-8pt}
\end{figure}


% describe LLM
Recently, \LLMs (LLMs) such as PaLM~\cite{chowdhery2022palm} and GPT family~\cite{brown2020language,ouyang2022training} %has been emerging substantial research interests
have revolutionized the methodology of tackling natural language processing (NLP) tasks
such as sentiment analysis~\cite{wankhade2022survey}, question answering~\cite{zaib2022conversational},  text summarization~\cite{yadav2022automatic}, and reasoning on arithmetic and common sense questions~\cite{zhao2023survey}. 

% describe LLM are very big
\LLMs (LLMs) are highly over-parameterized with millions or billions of parameters, e.g., the GPT-3 model has about 175 Billion parameters. Due to this redundancy in model design, LLMs can represent language in a highly flexible and expressive manner by capturing the complex and structured patterns in human languages. In addition, LLMs can generate remarkably natural dialogues and accurate answers with contextual understanding, sometimes even surpassing human experts in certain tasks. For example, in arithmetic reasoning, GPT-4 achieved an accuracy rate of 92\% on the GSM8K dataset~\cite{openai2023gpt4}; in common sense reasoning, KEAR achieved an accuracy rate of 89.4\% on the CSQA dataset~\cite{xu2022human}.

%With the advent of Chain-of-Thought and self-consistency, the performance of LLMs has seen a substantial improvement in the domains of arithmetic reasoning, common sense reasoning, and symbolic reasoning.

% describe a story
We consider a practical user scenario in which a large number of users can access a cloud-deployed LLM for solving personal tasks from all places over the world. For example, more and more primary school students and their parents rely on the 
capability of LLMs for solving mathematical problems. The users often access a LLM and ask common realistic questions. For example, primary school children might ask ``Chickens and rabbits are in the same cage, a total of 35 heads, 94 feet, how many chickens and rabbits are there?'', while computer science students often ask ``How to write a QuickSort in Python?''.


Due to the complexity in task understanding and reasoning, the LLMs often return the wrong answers even given seemingly simple questions. For example, on the GSM8K dataset, the fine-tuned GPT-3 (175B) with verifier only achieves an accuracy of 55.0\%. Meanwhile, the PaLM-540B (Few-shot-CoT) only achieves an accuracy of 58.1\%.~\cite{kojima2023large} 
\emph{How to improve the question answering accuracy has become a serious challenge which decides whether LLMs can be accepted as a robust and reliable part in realistic applications.}

One commonsense is that can we crowd-source many questions and aggregate those questions to better understand some common questions. A common question might be asked frequently as its variants in the concrete parameters or rephrased formulations. For example, the Chickens-and-rabbits questions can be asked with different number of heads and feet.
Now we want to ask \emph{Can we fully utilize those similar questions to improve the question answering of the LLMs without tuning the model parameters or infringing user privacy?}


% Recent progressives in \fdl (\textbf{FL})~\cite{fedavg} have proved that utilizing distributed data sources can both  preserve data privacy and enhance model training. 
% In the FL paradigm, each client trains a local learning model with \emph{own data}, while a central server regularly communicates with all agents to generate a better global model through the aggregation of the local models. 
%A key feature of FL is that no direct data exchange happens during the learning process, in contrast to centralized training.

In this study, we consider improving the reasoning capacity of LLMs by better understanding crowd-sourced similar questions, from which we can explore the contextual information and improve the LLM answers substantially. 
Inspired by FL, we propose two typical scenarios when a user sends a QA request to the LLM and the LLM tries to answer with a collected question database.
%\hl{Done:Xiangyang add your methodology, 3 types? or 2types?  Same formulation same parameters (SFSP-ZeroShot and SFSP-Cot), Same formulation different parameters (SFDP) ?}

\begin{itemize}[noitemsep,leftmargin=*]
\item \textbf{Synonymous Questions with Same Parameters (SP-questions)}. The cloud-deployed system retrieves from the database and finds several \synm but rephrased questions with exactly the same parameters. 
For example,\\
\emph{Q1:``If a farmer has a certain number of chickens and rabbits in a barn, and there are a total of 32 heads and 100 feet, how many chickens and how many rabbits does the farmer have?''\\
Q2:``In a barn, there are a certain number of chickens and rabbits that have a total of 32 heads and 100 feet.  how many of each animal are in the barn?''}

\item \textbf{Synonymous Questions with Different Parameters (DP-questions)}. This situation is harder as the question parameters mined in the database are different from each other. For example,\\
\emph{Q1:``If a farmer has a certain number of chickens and rabbits in a barn, and there are a total of 32 heads and 100 feet, how many chickens and how many rabbits does the farmer have?''\\
Q2:``A farmer has a total of 20 chickens and rabbits in his barn. If the total number of legs in the barn is 56, how many chickens and how many rabbits are in the barn?''}

\end{itemize}

For \textbf{SP-questions}, we propose to leverage LLMs to directly generate answers first. Then we federate the answers and apply the self-consistency~\cite{wang2023selfconsistency} technique to obtain the most voted answer for all \synm questions in the federation. We call this method \textbf{Fed-SP-SC} (Fed-SP with Self-Consistency). 

For \textbf{DP-questions}, we propose to leverage LLMs to generate consistent answers for each DP-questions first. Different from procedures of dealing SP-questions, we cannot directly agglomerate the answers since they are for different parameters. Instead, we federate them by forming the Chain-of-Thought (CoT) to provide hints to the LLMs. We append the original query to the CoT as the full prompt to obtain improved final answer. We call this technique \textbf{Fed-DP-CoT}.
 
 
Once the LLM has finished generating the answer using either Fed-SP-SC or  Fed-DP-CoT, the system will store both the questions and answers into the database. This enables the system to collect all records and leverage past records to produce re-fined answers to new queries. For questions that have been asked before with wrong answers, the system can evolve itself by correcting the  answers with self-consistency mechanism or with  more comprehensive CoT prompts.   


We extensively evaluate our methods on the GSM8K and SVAMP datasets and demonstrate that the Fed-SP-SC method achieves a notable improvement in accuracy of 14-18\% over the standalone LLMs with Zero-Shot-CoT (``Let's think step by step''). Additionally, our Fed-DP-CoT method delivers an impressive increase of 10-15\% over the standalone LLMs with Zero-Shot-CoT.
%\hl{Done: XIangyang. Not clear, this improvement is over Fed-SP-SC? or over what? what are the same conditions? Make this clear}.




We summarize our contributions in this study as follows. 
\begin{enumerate}[noitemsep,leftmargin=*]

%\hl{\{Done: modify. You may say:
% 1. We firstly propose two practical scenarios that ?
% 2. To tackle these scenarios, we propose a federated prompting and CoT ? to improve the query accuracy ?. 
% 3. Our methods can keep query private to other users, while getting benefits from distributed queries.\}}

%在特定的节日或者某一些领域，人们会经常问一些相同的或者相似的问题，这些问题可以通过聚合来为用户生成更好地答案；人们在对大语言模型prompt询问相同或相似的问题时会存在差异，这会使得大语言模型的回答侧重点不同，通过聚合这些问答过程可以让大语言模型回答相似的问题的时候更加全面。
% \item  In certain festivals or fields, people frequently ask the same or similar questions. By aggregating these questions, better answers can be generated for users. When people prompt the same or similar questions to LLMs, slight variations can result in differing answers. By aggregating these question-and-answer processes, the large language model can provide more comprehensive answers to similar questions.
\item We consider a practical but under-studied scenario, which is  the cloud-based LLMs are frequently asked similar and even \synm common questions from large number distributed users. 


%我们分别考虑相同问题和相似问题如何提升回答的准确性。我们采用Fed-SP-SC以提高相同参数的相同问题准确率，通过Fed-DP-CoT来提升不同参数的相似问题的准确性。
\item We abstract two main user scenarios: distributed users are querying synonymous questions that share the same parameters (SP-questions), and those that have different parameters (DP-questions).

\item We design the system to firstly federate those SP- and DP-questions first by retrieving the database. Then we propose to  utilize self-consistency methodology to select the most commonly voted answer to improve SP-question answering.  All consistent answers and CoTs will be stored back into database for further reuse.

% \item next, we design to amalgamate each SP-question's consistent answer to create a chain-of-thought for better DP-question answering. Our methods significantly improve answering quality rather than using Zero-shot prompting. We also design a simple disclaimer to better deal with noisy CoT generated from LLM answers without using ground truths.
\item We also amalgamate consistent answers to create a chain-of-thought prompt that significantly improves DP-questions answering quality.  We also design a simple disclaimer to handle noisy CoT generated from LLM answers better. 

%我们使用联邦学习来保护用户的隐私，这使得用户所问的问题对他人而说是不可见的。通过引入联邦学习，用户间可以共享与大语言模型之间的问答过程，以提升所有用户的体验
\item Inherited from Federated Learning, our Fed-SP-SC and Fed-DP-COT methods can collaboratively enhance the question-answering process of the LLM while preserving their anonymity. There would be no data exchange or leakage among distributed users.


\end{enumerate}




==> OK/tasks-05-04.tex <==
\section{Scenarios and Approaches}
\label{sec:tasks}

% In this section, we describe the practical scenarios can be seamlessly combined with AIGC to assist teachers in their classroom activities
%This section is organized as follows.
% In the previous section, we have discussed our envisioned overall AI model architecture called Dialogue Encoder (Dialogue-Enc), which is based on Large Language Models (LLMs). The D-Enc will help summarize the lengthy realistic teacher-student dialogue transcriptions. Then we introduce three realistic scenarios that could seamlessly incorporate AIGC for assisting teaching activities. 

In this section we present the realistic scenarios that can be seamlessly combined with AIGC to assist teachers in their classroom activities. Our proposed approaches aim to enhance the quality of instructional dialogues and facilitate constructive feedback for teachers.

%draw the architecture figure here

% 教案 -- AIGC生成问题 【案例】
% 补全 -- AIGC生成问题【案例】
% 标签 -- AI 分类问题 （提高精度？）
% 总结 -- Enc-Dec 提炼关键内容？
% 迁移 -- AIGC风格迁移 ？ 

% \subsection{Teaching Scheme AI Generation}
% % 教案生成
% The first practical user scenario we consider is as follows: Given an entire classroom dialogue, and our system can generate a teaching scheme for it.

% After obtaining the Answer-Sum through the \emph{Dialogue-Enc} method, we can fine-tune the generated teaching materials by providing specific prompts with defined formatting. For instance, we can specify the duration and teaching points to be included in the lesson plan, in order to achieve the desired outcome.

% % 提出相关能够提升效果的方法
% Our preliminary study shows that several novel methods, we proposed below, have been experimentally proven to be feasible and effective in improving results to a certain extent:


\subsection{Teacher-student Dialogue Auto-Completion}

% 对话补全
The first practical user scenario we consider is as follows: generating missing parts of classroom dialogue.

% 这里我们分为两种补全方式，一种是有Answer-Sum的，一种是没有教案的。
Here, we consider two different forms of input data: 

\begin{itemize}
    \item An entire classroom dialogue.
    \item A partial excerpt of the dialogue. 
\end{itemize}

We will describe specific methods for generating the necessary content for each form of input.

For the case of inputting the entire classroom dialogue, we can use the Dialogue-Enc method to obtain an Answer-Sum. Since lesson plans have structure and logical rigor, in order to improve the quality of the generated content, we first generate a lesson plan based on the Answer-Sum. Then, based on the divisions within the lesson plan, we generate the missing dialogue content for a particular section.

For the case of only having a partial excerpt of the classroom dialogue, we can still use the Dialogue-Enc method to obtain an Answer-Sum for the missing portion of the content. Similarly, we combine this incomplete Answer-Sum with a prompt to generate a complete lesson plan using LLM. Through multiple experiments, we found that the model automatically fills in the missing parts of the instructional process, and then follows the same method as above to generate the dialogue content by providing the lesson plan and the name or number of the section that needs to be completed.

We compared our approach with zero-shot, which is directly providing the connected dialogue content to LLM and prompting it to generate the middle dialogue. After analyzing the text generated by LLM under both approaches, we found that our proposed solution has advantages in accuracy, style similarity, and content saturation over the zero-shot approach.

% 提出相关能够提升效果的方法
Our preliminary study shows that the approaches, we propose as below, have been experimentally proven to be feasible and effective in improving results to a certain extent:

\begin{enumerate}[noitemsep,leftmargin=*]
\item \emph{Calling external APIs}. To complete missing classroom information, we generate teaching examples provided by the teacher using LLM and call external APIs to ensure that the corresponding example can obtain the correct answer. For instance, we can use the Wolfram API to calculate trigonometric function teaching examples provided by the teacher, to further improve the accuracy of the content.
\item \emph{Character Empowerment}. To guide the completion of dialogue contents, we can use role assignment to further tap into LLM's potential, such as prompting with "Suppose you are an elite teacher, please complete the classroom dialogue according to the content arrangement."
\item \emph{Contrastive Ranking}. When generating answers, learning the ability of contrastive ranking can help us search for other possible answers. We will discuss this in Sec.~\ref{sec:rlhf} in details.
\end{enumerate}

% \subsection{Teaching Style Transfer}
\subsection{Expert Teaching Knowledge and Style Transfer}
% 风格迁移，专家模仿

The second practical user scenario we consider is as follows: Given a data of classroom dialogue content, our system can perform style transfer based on user-specified classroom dialogue content.

% motivation
It is universally acknowledged that the process of developing a teacher's pedagogical abilities requires continuous imitation of successful teaching styles in order to enhance their own instructional capabilities. Whereas, given the limited number of expert classroom recordings available in the teaching dialogue database and the fact that the content taught by teachers often does not perfectly align with the themes covered by the expert recordings, utilizing AI to mimic the teaching styles of experts would yield a plethora of high-quality classroom dialogues for learning and reference purposes. Therefore, generating another similar-themed lesson plan and classroom dialogue content that mimics the given expert content would be highly meaningful and valuable.

However, the generation of the lesson plan by the LLM alone cannot directly produce the expected results. The difficulties we encounter in solving this task are summarized as follows:

\begin{enumerate}[noitemsep,leftmargin=*]
\item Insufficient understanding of existing lesson plans and  the distinct contents of two classes may lead to poor style transfer results. 
\item The generated results have limited style transfer ability and are unable to match the level of experts.
\end{enumerate}

Therefore, our task is to fully explore how to better understand the existing expert data and generate lesson plans and classroom dialogue content that meet human expectations for achievable style transfer effects. We first use the Dialogue-Enc method to obtain Answer-Sum, and then use it as a prompt to generate the corresponding lesson plan and classroom dialogue content.

% 这里我们分两种输入方式讨论，一种是有输入模板的，一种是zero-shot的。
Here, we consider two different forms of input data: 

\begin{itemize}
    \item Users are provided with the content of dialogue with master teachers in class.
    \item The user does not provide data and gives direct instructions.(zero-shot)
\end{itemize}

Our preliminary study has shown that the following methods have been experimentally proven to be effective, and can improve the results to some extent. And we will describe specific methods for generating the necessary content for each form of input.

For zero-shot user inquiries:
\begin{enumerate}[noitemsep,leftmargin=*]
\item \emph{Search-Semantic Matching}. Combining with proprietary databases and using Search-Semantic Matching can improve the credibility of generated results.
\item \emph{Chain-of-thought}. When a user initiates a query on our LLM systems, the system first performs Search-Semantic Matching. The proprietary database stores various templates in different styles, such as Tang poetry in Chinese language and arithmetic operations in mathematics. LLM automatically selects the best-matching template from the proprietary database based on its similarity and style. We then execute the CoT template. However, we consider a practical scenario where the matched best-style template may not always be optimal. We refer to these matches as "uncertain tags" since they cannot represent the true label. Therefore, we utilize the queries with uncertain labels together as CoT for the original query-question. Specifically, we use the user's inquiry and the previously-paired template as a prompt, followed by an error disclaimer at the end of this prompt, stating that "the provided template styles may not be fully applicable, please think more carefully." This complete prompt emphasizes that the templates suggested by LLM may not be entirely reasonable and may not be entirely imitated. Through preliminary experimentation, we have improved the effectiveness by using this method rather than directly providing templates. Finally, we attach the entire CoT as a prefix to the user's query prompt, allowing LLM to provide the final answer. 
\end{enumerate}

For inquiries that provide instructional content:
\begin{enumerate}[noitemsep,leftmargin=*]
\item \emph{Reinforcement Learning from Human Feedback}. Through continuous feedback from experts on the content generated by the LLM, its style transfer and content generation capabilities can be trained in a reverse manner. At the same time, the lesson plans generated by the LLM and the actual lesson plans designed by experts can be presented to other experts for evaluation, asking “Which group of lesson plans is more like the ones designed by expert teachers?”. If the results are “confused” and the difference in votes on each side is acceptable, then the results can be deemed acceptable. If the “confused” condition cannot be satisfied, then feedback should be given on the part of the lesson plan generated by the LLM that the experts do not view as being designed by expert teachers, providing a prompt such as “This lesson plan does not meet the requirements of style transfer to expert lesson plan, please generate a new one”, and continuing to generate new lesson plans.
\end{enumerate}

Intuitively, by utilizing the aforementioned methods to improve LLM content output, one can further enhance its style imitation ability and output effectiveness.

% maybe this is not a "task" for a subsection, but a section talking about evaluation and fine-tuning. Let's just put it here, and modify later.
%\subsection{Teaching Quality Grading and Model Fine-tuning}
%\subsection{Teaching Quality Grading}
\subsection{Assessment of AIGC for Classroom Teaching}

% 教案质量打分，人类干预
%The third practical user scenario we consider is as follows: given a classroom dialogue content data, our system can score the quality of the teaching plan and provide corresponding comments. However, simply instructing the LLM to generate score and comments that conform to expert evaluation standards is not effective. We summarize the difficulties to solve this task as follows:
The third practical user scenario we consider is to grade the AIGC for Education (AIGC-EDU) fairly and consistently. 
Two critical challenges that hinder the utilize of AIGC-EDU in realistic \ct is how to assess the quality of the generated content and how can it compare with human generated contents. 

% 描述三种打分方式 human feedback->LLMs->Ext-LLM
We envision and evaluate the following three types of methods of tackling the grading task in a fair and effective manner.

% \begin{enumerate}[noitemsep,leftmargin=*]
% \item Scoring is prone to inconsistent standards across different data, with significant differences between them.
% \item The comments provided are vague and lack specificity.
% \end{enumerate}

% Therefore, our task is to explore how to maximize the solution to the problem of inconsistent scoring standards and vague comments for different teaching plans. To this end, we propose several methods based on intervening measures to improve the output performance. Based on previous research, the effectiveness and applicability of these methods have been preliminarily verified and can improve the model’s generation effect to some extent. The following methods are proposed based on the Dialogue-Enc method for obtaining the Answer-Sum:

\subsubsection{Grading based on Human-Feedback.}
% 上述paper Section3.5, Eq(1) 附近，讲述了，如何sample pairwise的生成内容进行打分。
% 假设我们有N个AIGC教案，和M个人类专家教案，我们想进行打分

% \hl{TODO: here simply say, we can ask human pedagogical experts and senior teachers to provide their human evaluations on generated dialogues or contents. then we average the results for each content. then we emphasize its disadvantage: very costly since involves human feedback. cannot scale up like AIGC.}

We may seek the input of human pedagogical experts and senior teachers to evaluate the quality of our generated dialogues and content.
To avoid personal biases, we ensure that each teaching case is scored by multiple experts and calculate the final score for each case based on a reasonable set of scores or majority voting. 

The outcomes from this process are then averaged to obtain a final grade for each piece of content. Nevertheless, it is evident that this Human-Feedback based rating approach has a crucial drawback: it can be very costly since it requires human involvement. As a result, it cannot be easily scaled up in the same way as AIGC, and it is limited in its applicability.


\subsubsection{Grading based on LLMs.}
% \hl{Here we say we can ask LLMs themselves to grade, we call them self-ask.} 
As LLMs are versatile and capable language understanding models, they can grade their answers well, at least theoretically. We design the following method called Self-Ask~\cite{press2022measuring}(\emph{SA}) to achieve the self-grading. 

Concretely, for the generated answers of down-stream tasks, we add a prompting prefix such as "This is a self-generated result according to above dialogue. Can you grade its reasonable level from 1 (lowest) to 10 (highest) please? And can you justify why you give this score ?" We can fully automate this SA process and obtain a set of scores by assessing all answers in convenience.
% \hl{we emphasize its disavantage: not fine-tuned for educational purpose, so unreliable, and biased. especially for langauges other than English. then we say, we propose a novel method which trains on our self-collected proprietary classroom teaching dataset, as follows}

Nevertheless, SA still has systematic drawbacks. First of all, the general-purpose LLMs lack the background knowledge of those specific educational objectives. The decisions of grading answers could be based on general guesses such as the fluency of the dialogue but not based on \pedg reasons. Furthermore, it's a open secret that most LLMs are tuned better towards understanding English  contexts due to the dominating portion of English corpora for training. Thus, applying LLMs to grade the classroom teaching of Chinese poems and dramas could be seriously biased.

% , the application of this method is not fully satisfactory for languages other than English, especially in regards to achieving desired results. 

% . Although this approach significantly reduces the need for human involvement, it does not provide standards for LLMs. In other words, the fine-tuning process is not guided by , resulting in biased and unreliable outcomes. 



%which trains on our self-collected proprietary classroom teaching datasets, as follows.

% combine these three
\subsubsection{Grading and Commenting based on Ext-LLMs}. 
In view of the disadvantages of grading based on humans or general-purpose LLMs, we envision a novel methodology of training an External LLM (Ext-LLM) of mid-size for grading and commenting in this section.

We propose to utilize a mid-size pre-trained Ext-LLM with \emph{\textbf{supervised learning}} which we can fully control (store, fine-tune, and deploy) such as the commonly used Flan-T5~\cite{chung2022scaling} family from 80M to 11B parameters.
The motivation is to ensure the representative power of the Ext-LLM while maintaining the flexibility of fine-tuning and deploying with reasonable hardware requirements that academic institutes can afford.
% generates more persuasive results, achieving comparable performance with that of expert judgment. Below, we explain the training methods for scoring and commenting.

% 分数采用的是对比评分，利用奖励函数来促使其拟合
Now we explain how such an Ext-LLM can be tuned for grading purpose.
Inspired by the \emph{\textbf{Reward Modeling (RM)}} technique used for training InstructGPT~\cite{ouyang2022training},
we formulate the grading task as a supervised regression with ground-truth human evaluated grades, based on given dialogue as the contexts.
By comparing the AI-predicted and human evaluated ratings, the Ext-LLM can be adjusted as a reliable scoring model with human expertise from reward modeling as well as language understanding capability from pre-trained parameters with natural language understanding tasks.

% 评语采用CoT，树状模板链以促使其更深入理解教学案例，从而生成更好的评语
We can naturally extend the grading functionality to commenting the generated dialogues. As generating comments is indeed another AI-generation task, the Ext-LLM can naturally deal with it by learning from human examples. Here we assume that we have fine-tuned the commenting capability with realistic human evaluations.

We adopt the \emph{\textbf{Chain-of-Thought (CoT)}} method to guide the comment generation to ensure they are close to human expert evaluations.
To achieve this, we can attach a suffix to the generated content ``Therefore, assuming you are an elite teacher, please provide a professional evaluation given the dialogue.'' to provide the final comments. This procedure is also termed \emph{zero-shot CoT} that was initially used to improve reasoning performance~\cite{brown2020language}. We can also construct templates to utilize \emph{few-shot CoT} as ~\cite{brown2020language} in reasoning tasks.

%Firstly, we obtain a teaching case from user input and design a series of questions in conjunction with curriculum standards. To reduce token consumption and enhance specificity, we set the questions in a hierarchical chain format. In this way, Ext-LLMs can be more deeply guided to understand the teaching cases provided by the user, and all Q\& A pairs can be used as prompts. Finally, we append a suffix ``Therefore, assuming you are an educational practitioner, please provide a professional evaluation'' to provide the final answer.

% \textbf{Sub-Panel Evaluation} Combining key curriculum keywords further solidifies the scoring standards to avoid data bias. Several reference standards are given to score, such as the rationality of classroom structure and the innovation of teaching methods. They are scored separately, and the final score is obtained based on the weighted averages of each item.


% we should discuss this soon


% Note that the performance enhancement methods provided in the aforementioned scenarios are specific methods. In actual situations, they can be used in combination to achieve better results.


\section{AI Models Fine-tuning with Pedagogical Databases}
\label{sec:fine-tune}

% 在 conclusion 里面，我设想的是 Ext-LLMs 有这样的功能和优点
% 1. mid-size，并且完全可控, 对比之下商业的LLMs太大，私有，无法fine-tune
% 2. 保留了AIGC能力，又能在自有数据集上finetune，有可解释性，可用来打分，提供评价和矫正LLMs的输出，比如利用RLHF
%To enhance the interpretability and explainability of the black-box large AI models, we further propose to fully fine-tune a controllable and \hl{almost-deterministic} external LLMs. As the commercial LLMs are usually too huge and costly to fine-tune, and also are proprietary which prohibits the fully controlling. Thus, we proposed to employ mid-size Ext-LLMs to maintain the capacity of AIGC as well as the flexibility and interpretability. \hl{TODO} We train the Ext-LLMs to provide scores and comments for evaluation, and empower its correction capability of correcting LLMs outputs.



\subsection{Reinforcement Learning from Human Feedback}
\label{sec:rlhf}
% 我们对 N 和 M个教案，两两配对，生成一个 contrastive score, see InstructGPT paper.
Inspired by the supervised
\emph{Reward Modeling} methodology in InstructGPT~\cite{ouyang2022training}, we follow its contrastive ranking loss design to compare all pairs of AI-generated answers with human answers. Specifically, we select \emph{K} copies containing AI-generated and expert comments for each teaching case, and we make an arbitrary selection of these \emph{K} copies, two of which are selected as a pair each time, and then manually sorted for feedback. The specific loss function is as follows:

\begin{equation}
\operatorname{loss}(\theta)=-\frac{1}{\left(\begin{array}{c}
K \\
2
\end{array}\right)} E_{\left(x, y_w, y_l\right) \sim D}\left[\log \left(\sigma\left(r_\theta\left(x, y_w\right)-r_\theta\left(x, y_l\right)\right)\right)\right]
\end{equation}

where \emph{$r_\theta(x, y)$} is the scalar output of the reward model for prompt \emph{x} and completion \emph{y} with parameters
$\theta$, \emph{$y_{w}$} is the preferred completion out of the pair of \emph{$y_{w}$} and \emph{$y_{l}$}, and \emph{D} is the dataset of human comparisons.

\subsection{Ext-LLM Tuning}
% 我们这里主打 用了教学数据之后，LLM的可解释性， 比如输出comment，不在是一个黑盒子，而是可控的教学数据

% Through continuous human intervention and correction, the model can obtain more convincing results. When the model scores a user input teaching plan, it outputs the quality score and comments. CoT is used, and experts can guide its one-step correction based on a certain tree-like format with the generated comments, to achieve results that are similar to expert evaluation standards. Note that to ensure credibility, the experts referred to here are assumed to be multiple experts who evaluate simultaneously to avoid excessive individual differences.

We train Ext-LLM on our own educational dataset, and with constant human intervention and corrections, the model can obtain more convincing results. When the model scores the instructional plans entered by the user, it outputs evaluation scores and comments. Using CoT, the expert can be guided to make step-by-step corrections based on a certain tree format with the generated comments to achieve results that are similar to the expert evaluation criteria. It is important to note that the experts referred to here are assumed to be multiple experts evaluating at the same time in order to ensure credibility and to avoid excessive individual differences.

==> sections/experiments.tex <==
\section{Datasets}
\label{sec:dataset}

We make a comprehensive survey of EDU datasets and list here for readers' reference. According to their types, we provide four(?) categories as follows.

\subsection{Mathematics}

\textbf{Grade School Math (GSM8K)} is a math dataset with 7,473 training and 1,319 testing examples of grade-school-level word problems\cite{Cobbe2021TrainingVT}. These math problems typically require two to eight calculation steps to arrive at a final answer, as shown in Fig.\ref{fig:Fed-SC}. GSM8K is widely used as a benchmark dataset for testing the arithmetic and commonsense reasoning capacities of LLMs~\cite{huang2022large, kojima2023large}.

\textbf{Simple Variations on Arithmetic Math word Problems (SVAMP)} is a dataset of simple arithmetic math word problems~\cite{patel2021nlp} with around 6,000 samples. Each data instance has a short story and a question about unknown quantities. SVAMP provides a benchmark test set for comparing the textual understanding and reasoning abilities of LLMs, which is widely compared in recent studies~\cite{patel2021nlp, wei2022chain, wang2023selfconsistency}.

\subsection{Reasoning}







